Uncertainty-Aware Adaptive Dynamics For Underwater Vehicle-Manipulator Robots

Accurate and adaptive dynamic models are critical for underwater vehicle-manipulator systems where hydrodynamic effects induce time-varying parameters. This paper introduces a novel uncertainty-aware adaptive dynamics model framework that remains linear in lumped vehicle and manipulator parameters, and embeds convex physical consistency constraints during online estimation. Moving horizon estimation is used to stack horizon regressors, enforce realizable inertia, damping, friction, and hydrostatics, and quantify uncertainty from parameter evolution. Experiments on a BlueROV2 Heavy with a 4-DOF manipulator demonstrate rapid convergence and calibrated predictions. Manipulator fits achieve R2 = 0.88 to 0.98 with slopes near unity, while vehicle surge, heave, and roll are reproduced with good fidelity under stronger coupling and noise. Median solver time is approximately 0.023 s per update, confirming online feasibility. A comparison against a fixed parameter model shows consistent reductions in MAE and RMSE across degrees of freedom. Results indicate physically plausible parameters and confidence intervals with near 100% coverage, enabling reliable feedforward control and simulation in underwater environments.

==> sections/Notation.tex <==
\section{Notations and Conventions}
\label{sec:notation}


==> sections/Research_Objective.tex <==
\section{Research Objectives}
% The objective of this study is to develop an adaptive dynamics formulation for free-floating underwater manipulators, enabling the model to accurately predict future states under uncertain conditions. This model will incorporate hydrodynamic forces acting on each rigid body in the system and the effects of rotor dynamics within the manipulator joints. The time-varying parameters will be updated during operation, allowing the system to rapidly adapt to environmental changes and improve prediction accuracy.
